Data-driven modelling of turbine wake interactions and flow resistance in large wind farms

Turbine wake and local blockage effects are known to alter wind farm power production in two different ways: (1) by changing the wind speed locally in front of each turbine; and (2) by changing the overall flow resistance in the farm and thus the so-called farm blockage effect. To better predict these effects with low computational costs, we develop data-driven emulators of the `local' or `internal' turbine thrust coefficient $C_T^*$ as a function of turbine layout. We train the model using a multi-fidelity Gaussian Process (GP) regression with a combination of low (engineering wake model) and high-fidelity (Large-Eddy Simulations) simulations of farms with different layouts and wind directions. A large set of low-fidelity data speeds up the learning process and the high-fidelity data ensures a high accuracy. The trained multi-fidelity GP model is shown to give more accurate predictions of $C_T^*$ compared to a standard (single-fidelity) GP regression applied only to a limited set of high-fidelity data. We also use the multi-fidelity GP model of $C_T^*$ with the two-scale momentum theory (Nishino \& Dunstan 2020, J. Fluid Mech. 894, A2) to demonstrate that the model can be used to give fast and accurate predictions of large wind farm performance under various mesoscale atmospheric conditions. This new approach could be beneficial for improving annual energy production (AEP) calculations and farm optimisation in the future.

==> Lato-fonts/Makefile <==
## Makefile
## Copyright 2011 Mohamed El Morabity
#
# This work may be distributed and/or modified under the conditions of the LaTeX
# Project Public License, either version 1.3 of this license or (at your option)
# any later version. The latest version of this license is in
# http://www.latex-project.org/lppl.txt and version 1.3 or later is part of all
# distributions of LaTeX version 2005/12/01 or later.
#
# This work has the LPPL maintenance status `maintained'.
#
# The Current Maintainer of this work is Mohamed El Morabity
#
# This work consists of all files listed in manifest.txt.

######################
# Fonts informations #
######################

FONT_NAME = lato
FOUNDRY = public
FONT_CODES = fla

# Supported LaTeX encodings
SUPPORTED_ENCODINGS = ot1 t1 ts1
# Supported LaTeX encodings containing small caps
SUPPORTED_SC_ENCODINGS = $(filter-out ts1,$(SUPPORTED_ENCODINGS))
# Custom encodings provided
INPUT_ENCODINGS = $(INPUT_ETX_FILES:$(FONT_NAME)-%.etx=%)


#####################
# Installation root #
#####################

TEXMFHOME = $(shell kpsexpand '$$TEXMFHOME')


###########
# Archive #
###########

ARCHIVE_ROOT = $(FONT_NAME)
ARCHIVE = $(FONT_NAME).zip


###########
# Sources #
###########

TRUETYPE_FILES = $(wildcard *.ttf)

# Fontinst files
FONTINST_FILE = $(FONT_NAME)-drv.tex
FONTINST_MAP_FILE = $(FONT_NAME)-map.tex

# Custom Fontinst encoding files
INPUT_ETX_FILES = $(FONT_NAME)-01.etx $(FONT_NAME)-02.etx $(FONT_NAME)-dotlessj.etx
MTX_FILES = $(FONT_NAME)-fixlatin.mtx $(FONT_NAME)-fixtextcomp.mtx

STYLE_FILES = $(wildcard *.sty)

DOCUMENTATION = $(FONT_NAME).tex $(FONT_NAME).pdf $(FONT_NAME)-samples.tex $(FONT_NAME)-samples.pdf README CHANGES

# Files to be installed in texmf/source
SOURCE_FILES = $(FONTINST_FILE) $(FONTINST_MAP_FILE) $(INPUT_ETX_FILES) $(MTX_FILES) Makefile ttf2type1.pe


###################
# Generated files #
###################

TYPE1_FILES = $(TRUETYPE_FILES:.ttf=.pfb) $(TRUETYPE_FILES:.ttf=-LCDFJ.pfb)
AFM_FILES = $(TYPE1_FILES:.pfb=.afm)

# Fontinst log file
FONTINST_REC_FILE = $(FONT_NAME)-rec.tex

# Metrics files
PL_FILES = $(foreach e,$(INPUT_ENCODINGS),   \
             $(TRUETYPE_FILES:.ttf=-$(e).pl) \
           )
OUTPUT_MTX_FILES = $(PL_FILES:.pl=.mtx)
VPL_FILES = $(foreach e,$(SUPPORTED_ENCODINGS),          \
              $(TRUETYPE_FILES:.ttf=-$(e).vpl)           \
            )                                            \
            $(foreach e,$(SUPPORTED_SC_ENCODINGS),       \
              $(TRUETYPE_FILES:.ttf=-SmallCaps-$(e).vpl) \
            )
TFM_FILES = $(PL_FILES:.pl=.tfm) $(VPL_FILES:.vpl=.tfm)
VF_FILES = $(VPL_FILES:.vpl=.vf)

MAP = $(FONT_NAME).map

# Font definition files
FD_FILES = $(foreach e,$(SUPPORTED_ENCODINGS), \
             $(foreach f,$(FONT_CODES),        \
               $(e)$(f).fd                     \
             )                                 \
           )

# Generated encoding files
ENC_FILES = $(INPUT_ETX_FILES:.etx=.enc)

# Generated files to be installed
GENERATED_FILES = $(TYPE1_FILES) $(AFM_FILES) $(TFM_FILES) $(VF_FILES) $(MAP) $(FD_FILES) $(ENC_FILES)


default: all


all: dist


dist: $(ARCHIVE)


%.pfb %.afm: %.ttf
	fontforge ttf2type1.pe $<
	# BUGFIX: fix FontName to the name of the file
	sed -i "s/^FontName .*/FontName $*/" $*.afm


%-LCDFJ.pfb: %.pfb
	t1dotlessj $< $@


%-LCDFJ.afm: %-LCDFJ.pfb
	pf2afm $<
	# BUGFIX: fix FontName to the name of the file
	sed -i "s/^FontName .*/FontName $*/" $*.afm


%.tfm: %.pl
	pltotf $< $@


%.tfm: %.vpl
	vptovf $^ $


%.vf: %.vpl
	vptovf $^ $@


$(FONTINST_REC_FILE): $(AFM_FILES) $(MTX_FILES) $(FONTINST_FILE)
	latex $(FONTINST_FILE)


$(PL_FILES) $(VPL_FILES): $(FONTINST_REC_FILE)


$(MAP): $(FONTINST_REC_FILE) $(FONTINST_MAP_FILE)
	latex $(FONTINST_MAP_FILE)


$(FD_FILES) $(ENC_FILES): $(MAP)


texmf-tree: clean-texmf-tree $(GENERATED_FILES) $(SOURCES_FILES)
	mkdir -p $(ARCHIVE_ROOT)/doc/fonts/$(FONT_NAME)/
	mkdir -p $(ARCHIVE_ROOT)/tex/latex/$(FONT_NAME)/
	mkdir -p $(ARCHIVE_ROOT)/fonts/{enc,map}/dvips/$(FONT_NAME)/
	mkdir -p $(ARCHIVE_ROOT)/fonts/{afm,tfm,truetype,type1,vf}/$(FOUNDRY)/$(FONT_NAME)/
	mkdir -p $(ARCHIVE_ROOT)/source/fonts/$(FONT_NAME)/
	cp -p $(DOCUMENTATION) $(ARCHIVE_ROOT)/doc/fonts/$(FONT_NAME)/
	cp -p $(FD_FILES) $(STYLE_FILES) $(ARCHIVE_ROOT)/tex/latex/$(FONT_NAME)/
	cp -p $(ENC_FILES) $(ARCHIVE_ROOT)/fonts/enc/dvips/$(FONT_NAME)/
	cp -p $(MAP) $(ARCHIVE_ROOT)/fonts/map/dvips/$(FONT_NAME)/
	cp -p $(AFM_FILES) $(ARCHIVE_ROOT)/fonts/afm/$(FOUNDRY)/$(FONT_NAME)/
	cp -p $(TFM_FILES) $(ARCHIVE_ROOT)/fonts/tfm/$(FOUNDRY)/$(FONT_NAME)/
	cp -p $(TRUETYPE_FILES) $(ARCHIVE_ROOT)/fonts/truetype/$(FOUNDRY)/$(FONT_NAME)/
	cp -p $(TYPE1_FILES) $(ARCHIVE_ROOT)/fonts/type1/$(FOUNDRY)/$(FONT_NAME)/
	cp -p $(VF_FILES) $(ARCHIVE_ROOT)/fonts/vf/$(FOUNDRY)/$(FONT_NAME)/
	cp -p $(SOURCE_FILES) $(ARCHIVE_ROOT)/source/fonts/$(FONT_NAME)/
	cp -p README $(ARCHIVE_ROOT)
	cd $(ARCHIVE_ROOT) && find . -type f > manifest.txt


$(ARCHIVE): clean-texmf-tree texmf-tree
	zip -r $@ $(ARCHIVE_ROOT)


install: texmf-tree
	mkdir -p $(TEXMFHOME)
	cp -a $(ARCHIVE_ROOT)/* $(TEXMFHOME)
	texhash
	updmap --enable Map=$(MAP)


uninstall:
	$(RM) -r $(TEXMFHOME)/doc/latex/$(FONT_NAME)/
	$(RM) -r $(TEXMFHOME)/tex/latex/$(FONT_NAME)/
	$(RM) -r $(TEXMFHOME)/fonts/{enc,map}/dvips/$(FONT_NAME)/
	$(RM) -r $(TEXMFHOME)/fonts/{afm,tfm,type1,vf}/$(FOUNDRY)/$(FONT_NAME)/
	$(RM) -r $(TEXMFHOME)/source/$(FONT_NAME)/
	updmap --disable $(MAP)
	texhash


clean: clean-texmf-tree
	$(RM) $(TYPE1_FILES) $(AFM_FILES)
	$(RM) $(FONTINST_REC_FILE)
	$(RM) $(PL_FILES) $(TYPE1_FILES:.pfb=.pl)
	$(RM) $(OUTPUT_MTX_FILES) $(TYPE1_FILES:.pfb=.mtx)
	$(RM) $(VPL_FILES)
	$(RM) $(TFM_FILES)
	$(RM) $(VF_FILES)
	$(RM) $(MAP)
	$(RM) $(FD_FILES)
	$(RM) $(ENC_FILES)
	$(RM) $(ARCHIVE)
	$(RM) *~ *.log


clean-texmf-tree:
	$(RM) -r $(ARCHIVE_ROOT)


.PHONY: clean clean-texmf-tree texmf-tree

